ScalOTA: Scalable Secure Over-the-Air Software Updates for Vehicles

Over-the-Air (OTA) software updates are becoming essential for electric/electronic vehicle architectures in order to reduce recalls amid the increasing software bugs and vulnerabilities. Current OTA update architectures rely heavily on direct cellular repository-to-vehicle links, which makes the repository a communication bottleneck, and increases the cellular bandwidth utilization cost as well as the software download latency. In this paper, we introduce ScalOTA, an end-to-end scalable OTA software update architecture and secure protocol for modern vehicles. For the first time, we propose using a network of update stations, as part of Electric Vehicle charging stations, to boost the download speed through these stations, and reduce the cellular bandwidth overhead significantly. Our formalized OTA update protocol ensures proven end-to-end chain-of-trust including all stakeholders: manufacturer, suppliers, update stations, and all layers of in-vehicle Electric Control Units (ECUs). The empirical evaluation shows that ScalOTA reduces the bandwidth utilization and download latency up to an order of magnitude compared with current OTA update systems.

==> arch.tex <==
\section{\acronym Architecture and Protocol}
\label{sec:arch}

\subsection{Symbols}
TODO: we keep adding symbols here as we go.
\todo{I need a symbol for an "update list", i.e., a list of packages a vehicle shall install. The name can be improved.}
\todo{I need a symbol for delegation.}
\todo{I need a symbol for metadata.}

A software update $\Delta$ is composed of an ordered list of fine-grained data differential \textit{chunks} $\delta$, and represented as $\Delta=(\delta_1,\delta_2,...,\delta_m)$. An update message $M$ with payload $\Delta$, version $v$, tagged with timestamp $t$, and destined to a designated ECU $e$ is represented as $M=(\Delta, v, t, e)$. A message $M$ can be signed digitally by sender $i$ to ensure authenticity and integrity, and is thus denoted by  $\langle M \rangle_i = \langle \Delta, v, t, e\rangle_i$.


\begin{center}
\begin{tabular}{||c c||} 
 \hline
 Symbol & Meaning\\ [0.5ex] 
 \hline\hline
 $\Delta$ & software update \\ 
 $\delta$ & software update chunk \\ 
  $X$ & Manifest \\
  $v$ & version\\
  $t$ & timestamp \\
  $e$ & ECU \\
  $n$ & delegation \\
  $m(v, e)$ & metadata for update $v$ of ecu $e$ \\
 $\langle\rangle_i$ & signed payload by $i$ \\
 \hline
\end{tabular}
\end{center}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{arch}
\caption{The \acronym architecture. A supplier (e.g., Tier 1) produces updates and notifies the OEM. The latter bundles and update metadata with required keys, signatures, and dependencies using the information from the OEM's fleet inventory and time standard server. An EV update station subscribes to the OEM package manager to receive updates corresponding to fleet vehicles in the region. The station downloads the update images via the supplier's image servers after correct delegations. Updates follow a fine-grained tagging scheme to avoid downloading duplicate updates for the same auto part potentially used in several models or brands.}
\label{fig:OTA-arch}
\end{figure*}


\subsection{Overview}
Figure~\ref{fig:OTA-arch} depicts the architecture of \acronym. The architecture is composed of four main parts: the manufacturer's Software Update Director (SUD), the supplier chain of Image Repositories, the  Update Distribution Broker (UDB), and the vehicles. 

%\textbf{Software Update Director (SUD).} The role of the manufacturer SUD is to control the updates of the entire fleet and maintain the updates through the suppliers. For this, the SUD retains an inventory database of the entire fleet information and vehicles specifications, versions, and associated suppliers. The software updates, package dependencies (of different ECUs' software), and the timestamps are all secured through signed manifests with dedicated and redundant cryptographic keys to ensure an end-to-end chain of trust. This is crucial to defend and mitigate more than dozen attacks as mentioned in the threat model, and detailed later in Section~\ref{}. The SUD includes a store for Image Repositories that could retain small software images or simply references to outsourced suppliers.  The SUD communicates with the fleet to push the software updates timely through the Update Update Distribution Broker (UDB) or directly to vehicles through an MQTT publish/subscribe protocol. 

\textbf{Software Update Director (SUD).} The role of the manufacturer SUD is to control the updates of the entire fleet. For this, the SUD retains an inventory database of the entire fleet information and vehicle specifications, versions, and associated suppliers. The SUD uses state-of-the-art techniques to calculate version dependencies and conflicts to generate safe update lists. The SUD contains roles, which represents entities inside the SUD with different responsibilities; when a role writes metadata it always signs it with its own key(s). The roles are: timestamp---responsible for applying timestamps to the SUD's metadata; targets---stores the various updates' information; snapshot---creates metadata describing stable software bundles; and root---when the SUD writes a manifest it is signed by this role, i.e., the manifest may include elements from other roles, but the root signs on top of everyone else.

\textbf{Image Repository (IR).} This is a database where all of an OEM-associated software is stored, including packages developed in-house and from \textit{N}-Tier suppliers. The packages developed by the OEM are directly signed by it, using a set of keys related to the OEM's developer team. When the suppliers create a new software update $\Delta$ with version $v$, they sign it to generate $\langle \Delta \rangle_i$, generate metadata $m(v, e)$ about it (e.g., dependencies and conflicts, version), and then place $[\langle \Delta \rangle_i, m(v, e)]$ in the OEM's IR. This creates a delegation; the OEM stores some $\Delta$ that it not developed, will sign manifests that mention $\Delta$ and its metadata, but the responsible for $\Delta$ and all security around it is the supplier.

\textbf{The Update Distribution Broker (UDB).} The UDB is composed of an Update Engine (UE) and a a distributed network of vehicle update stations (UStations), e.g., associated with EV charging stations. Each UStation collects identifiers about vehicle models in its corresponding zone, for which updates are downloaded and cached. The UStation pulls from the UE updates corresponding to the identifier, that by its turn subscribes to the corresponding updates provided by the manufacturer's SUD, through the MQTT pub/sub protocol. The UE then redirect the update downloads to the designated UStation. The UE can optimize the cache of the software updates on zonal-basis. It can also predict update usage, i.e., if an update $\Delta$ becomes available for a vehicle type that is frequently seen in its UStations, then it can preemptively publish it.

\textbf{Vehicle.} The vehicles are composed of a primary and several secondary ECUs, for which software updates are continuously needed. The vehicle learns about new updates only by querying the OEM's SUD. The software images can downloaded via the OEM's IR or through the UStations for faster and more efficient bandwidth utilization. 

\textbf{Supplier.} The suppliers produce and package the update images of each autopart, tag them by model and manufacturer, and store them in local or manufacturer's Image Repository. As explained later, a direct supplier (called Tier1) can securely delegate software to other third-party (Tier 2 or Tier 3) suppliers.

\textbf{Manifests.} These are tree metadata structures used in the various parts of the protocol. The the root node identifies the creator of the manifest; nodes and leafs vary according to context and are described when presented. Once finalised, all manifests are signed by its creator.

\subsection{Update Protocol}

\subsubsection{Initialization}
Before dispatching a vehicle to the market, an OEM installs the most recent software versions for all of its parts. The vehicle's model and parts are known by its unique \textit{Vehicle Identification Number (VIN)}, composed of 17 characters. In particular, the very first 11 characters, we call them \textit{Model Identification Number (MIN)}, defines the corresponding features, specifications, and manufacturer. To keep the vehicle in circulation up-to-date, the OEM retains update meta-data in the SUD's fleet inventory, namely:
\begin{itemize}
    \item the VIN,
    \item the MIN and a list of soft parts with associated suppliers, and
    \item the software update info.: last available version, associated package dependencies and conflicts, and packaging datetime.
\end{itemize}

\subsubsection{Packaging and Roll-out}
When the suppliers publish updates for their ECUs to the Image Repository (due to an identified bug or to provide a new feature), they also push to the OEM a manifest describing the new software (manifests are described in Section\ref{}), and the software's dependencies. 
Based on this information, the OEM takes two actions.
First, it packages the new update including the possible dependencies as update prerequisites to resolve any conflicts with other software. This information is added to the SUD, which then guarantees that a new software update contains or enforces all other necessary requirements.
Second, it updates the roles involved with updates, namely targets and snapshot.
At this stage, the UDB can push new manifests to the subscribers.
Finally, when an authorized user $u$ queries regarding new updates, the SUD creates a manifest designed for $u$ describing what packages it should download. This manifest is generated live and is signed by all roles to create a robust trust-chain for integrity and authentication.

\subsubsection{Downloading Updates from UStation}
A vehicle owner previously obtained a software update service account from the UDB to maintain its vehicle up-to-date in circulation.
%The UDB provides a list of supported UStations and corresponding authentication keys that the vehicle can get updates from.
When the vehicle connects to the UStation it authenticates it as an authorized edge update provider; otherwise, it aborts the process.
First, the vehicle downloads a fresh manifest from the UDB to get information about updates for its ECUs.
%Before connecting to a UStation $S$ to download updates, the vehicle downloads from the Director Server a manifest describing any novel software versions.
%Then, while connected to the station, e.g., while recharging at an integrated EV-UStation, it connects to the UStation via wired connection. 
%It authenticates to the UStation and checks for any new updates described in the director's manifest to download them.
Then, assuming it has updates to download and install, it queries the UStation for these updates,
There are three cases: update Hit, Miss, or Unknown.
\begin{description}
    \item[Hit:] the UStation has local caches for the required updates. %newer updates than the versions of the corresponding vehicle (verified via the VIN).
    This means that the UDB pushed the updates to this UStation, or that a previous access to this UStation had occurred by a vehicle requiring ths same software. The vehicle's primary then downloads the software packages (i.e., all dependencies) of the software updates to be installed.
    \item[Miss:] the UStation does not have the packages requested by the vehicle. In this case, the UStation will pull updates from the UE. The UE sends an update link to download the update from the corresponding Image Repository. The UE sends a security token each time a down is requested by a UStation.
    \item[Unknown:] the current vehicle MID is unknown to the UStation $S$, i.e., have not been seen before. In this case, the UStation sends a subscribe request to the UE. If the latter has the MID subscription through another UStation $Z$ it adds $S$ to its list of destinations and pushes updates about this MID as above (by sending a download link and corresponding credentials). On the other hand, if the UE does not know about the MID at all, it subscribes to the OEM's SUD and starts getting meta-data updates about this model. This meta-data is then used to pull updates from Image Repositories as above.
\end{description}

\subsubsection{Pushing updates to Secondaries}
Pushing update from primaries to secondaries is key in automotive software updates. The role of a primary is essential in the process since the corresponding ECU has typically higher capacity (memory, bandwidth, and processing) than secondary constrained ECUs. On the other hand, given that a modern vehicle can have more than 100 ECUs, having each handling the update independently with the OEM SUD would be a very complex and costly task. Given this, there are two cases for pushing the updates from the primary to a secondary ECU considering the trust model.

\textbf{Trusted Primary.} Assuming the primary is trusted, it can handle the entire software download process, full verification (as specified in Section?), and delivery to the secondary ECU. The secondary on the other hand can have (1) a software update/flashing tool that could be executed directly remotely by the primary (e.g., in an RPC style), or (2) a running a flashing service process that can be invoked to the the update and flashing locally. In either case, the secondary does not have to verify the received updates via the trusted primary (although it should do a basic sanity check, e.g., error correction or erasure code). It would rather do a partial verification (as explained in section?). 

\textbf{Untrusted Primary.} An untrusted primary may lead to integrity or availability issues (and confidentiality if considered). It could violate integrity by forging the software update packages (i.e., updates and manifests). This would require the secondary to do a full verification for the updates. On the other hand, the primary may simply delay or drop the updates destined to the secondary. To address this, a secondary's flashing service (i.e., periodic process) should handle the communication with the primary, which can no longer enforce update remotely. The flashing service has two main roles. The first is to request an \textit{update report} from the primary upon each vehicle ignition. The primary should reply (within a given time delay) with a signed message from the OEM, specifying the last available software version for the corresponding secondary ECU. These two roles ensure that the primary could neither delay or discard the received updates from the OEM beyond the pr-defined period (.e.g, defined on safety basis), nor tampering with their content. If these conditions are unmet, the secondary sends an alert message to the driver or OEM, e.g., via displaying an alert message on the headset or beeping. 

QUESTION: after pushing, there is flashing. If some ECU failed and there are dependencies, there others should roll-back. This needs some atomic broadcast protocol to be done well. What is your take?

\subsection{Extensions}
\subsubsection{Adding/removing a UStation}
The UDB should be able to scale-out and scale-in over time. This is done by adding new UStations or removing others occasionally or permanently, e.g., in the case of a "retired" UStation. The main incentives are referred to business, convenience, and performance reasons. Nevertheless, denouncing some UStations may be driven by security threats which requires putting the UStation out of service. 

Technically, when adding a new UStation, it gets assigned an identifier and a security authentication key, i.e., a certificate. This is needed to ensure that the vehicles authenticate to approved and trusted UStations, through which software updates are downloaded. A UStation that is under threat can get its certificate revoked and the key is added to the UDB Certificate Revocation List (CRL), that is always updated and sent to the vehicles. Vehicles are then protected since software updates can no longer be validated. 

\subsubsection{Incremental updates}
In modern vehicles, the software update footprint can be very large (e.g., up to 1 GB). In this case, not all updates are expected to be fully downloaded at a UStation. To the contrary, the vehicle should be able to continue downloading the update remainder (to reduce bandwidth, time, and energy waste) through other means, e.g., another UStation or directly through the OEM via a cellular or 5G connection. For this, updates can be packaged as a series of fine-grained ordered \textit{buckets}. A download that is interrupted at some bucket could easily continue the download from the failed bucket forward, until the complete package is downloaded. The primary verifies this after the download is complete by checking the digest of the the full package across the assembled one of the ordered buckets downloaded. This ensures that no buckets but the correct ones are added in their specific order.   

\subsubsection{Reducing Misses}

One of the properties of \acronym is reducing the update time. This is salient in the case of cache hit since the update is at the closest proximity to the vehicle. However, under cache hits, the update time will be higher since the UStation should get the update throughout the UDB while the vehicle is waiting for the update at the station. While 
having a decent cache storage capacity can reduce the cache misses, software update cannot be afforded at scale. On the other hand, a newly added UStation would suffer a lot of cache misses. 

To address this, we propose a proactive technique to speculate the needed updates at a new UStation A or pushing updates for new vehicles even if they have not been requested by an existing UStation. This technique is based on filling A's cache using the cache of the k $l$-hop closest UStations, where $l \in \mathbb{N}$. The intuition is that it is likely that vehicle models circulating in the proximity of A are significantly similar to those already passed by the neighbouring k USations. Therefore, the UDB engine UE computes a list of the cardinally of the MIDs at the k UStations. The highest the cardinally the more abundant a associated model is in a zone. The UE then sends the list to  UStation A that proactively initiates downloading the updates starting with the the highest carnality MIDs, and until the cache is full. Although this technique improves the hit rate much better than an empty cache, an interesting research is to study more intelligent ML-based recommender systems, based on the traffic at the neighbours and trajectories patterns.







==> arch2.tex <==
\section{\acronym Architecture and Protocol}
\label{sec:arch}

\subsection{Manifests and Symbols}

%A software update $\Delta$ is composed of an ordered list of fine-grained data differential \textit{chunks} $\delta$, and represented as $\Delta=(\delta_1,\delta_2,...,\delta_m)$. An update message $M$ with payload $\Delta$, version $v$, tagged with timestamp $t$, and destined to a designated ECU $e$ is represented as $M=(\Delta, v, t, e)$. A message $M$ can be signed digitally by sender $i$ to ensure authenticity and integrity, and is thus denoted by  $\langle M \rangle_i = \langle \Delta, v, t, e\rangle_i$.

A software update $\Delta$ is composed of an ordered list of fine-grained data differential \textit{chunks} $\delta$, and represented as $\Delta=(\delta_1,\delta_2,...,\delta_m)$.
Metadata is exchanged between entities during various protocol steps using manifests, represented as $X=(PB,S)$, where $PB$ is the payload block of the manifest, and $S$ is a list of signatures of $PB$.
$PB$ is represented as $PB=(p,c)$, where $p$ is the actual payload, and $c=(t,v,r)$ is metadata of the payload, composed of a timestamp $t$, a manifest version $v$, and the certificate of the signer $r$.
The most common type of manifest payload is metadata $p=(f_\Delta,l_\Delta,h_\Delta,v_\Delta,e)$ about an update $\Delta$, where $f$ is the filename, $l$ is the file length, $h$ is the hash, $v$ is the version, and $e$ is the target ECU.
This payload can be extended to include a list of $\Delta$'s dependencies $d$ and conflicts $cf$, thus becoming $p=(f_\Delta,l_\Delta,h_\Delta,v_\Delta,e,d,cf)$.
If the payload describes a list of updates, it is represented as $[p]$ as a contraction of $(p_1,p_2,...,p_n)$.
Other payloads are described in the paper when appropriate.
The signature list $S=((s_1,sp_1),(s_2,sp_2),...,(s_n,sp_n))$ is a list of pairs $(s,sp)$, where $sp$ is the protocol used to produce $s$.
For simplification, we represent $S$ as $\langle PB\rangle_{i}$, meaning that entity $i$ created a signature list $S$ by signing $PB$.
These symbols are summarized on Table~\ref{tab:symbols}.

\begin{table}[t]
\center
    \caption{List of most used symbols in the manifests and protocols.}
    \label{tab:symbols}
    
\begin{tabular}{c|c} 
 \toprule
 Symbol & Meaning\\ [0.5ex] 
 \midrule
 $\Delta$ & Software update \\ 
 $\delta$ & Software update chunk \\ 
  $X$ & Manifest \\
  $v$ & Version\\
  $t$ & Timestamp \\
  $e$ & ECU \\
  $PB$ & Payload block \\
  $p$ & Payload \\
  $[p]$ & List of payloads \\
  $c$ & Metadata of payload \\
  $S$ & Signature list \\
  $h_\alpha$ & Hash of $\alpha$ \\
  $n$ & Delegation \\
  $r_i$ & Certificate of $i$ \\
 $\langle P\rangle_i$ & $i$'s signature of $P$ \\
 \bottomrule
\end{tabular}
\end{table}

%Full manifest
% $X=(PB,\langle PB\rangle_{signer}), PB=((f_\Delta,l_\Delta,h_\Delta,v_\Delta,e,d,cf),(t,v,r))$

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{arch}
\caption{The \acronym architecture. A supplier (e.g., Tier 1) produces updates and notifies the OEM. The latter bundles and update metadata with required keys, signatures, and dependencies using the information from the OEM's fleet inventory and time standard server. An EV update station subscribes to the OEM package manager to receive updates corresponding to fleet vehicles in the region. The station downloads the update images via the supplier's image servers after correct delegations. Updates follow a fine-grained tagging scheme to avoid downloading duplicate updates for the same auto part potentially used in several models or brands.}
\label{fig:OTA-arch}
\end{figure*}


\subsection{Architecture overview}
Figure~\ref{fig:OTA-arch} depicts the architecture of \acronym. The architecture is composed of four main parts: the manufacturer's Software Update Director (SUD), the supplier chain of Image Repositories, the EV Station Manager (ESM), and the vehicles. 

%\textbf{Software Update Director (SUD).} The role of the manufacturer SUD is to control the updates of the entire fleet and maintain the updates through the suppliers. For this, the SUD retains an inventory database of the entire fleet information and vehicles specifications, versions, and associated suppliers. The software updates, package dependencies (of different ECUs' software), and the timestamps are all secured through signed manifests with dedicated and redundant cryptographic keys to ensure an end-to-end chain of trust. This is crucial to defend and mitigate more than dozen attacks as mentioned in the threat model, and detailed later in Section~\ref{}. The SUD includes a store for Image Repositories that could retain small software images or simply references to outsourced suppliers.  The SUD communicates with the fleet to push the software updates timely through the Update Update Distribution Broker (UDB) or directly to vehicles through an MQTT publish/subscribe protocol. 

\textbf{Software Update Director (SUD).} The role of the manufacturer SUD is to control the updates of the entire fleet. For this, the SUD retains an inventory database of the entire fleet information and vehicle specifications, versions, and associated suppliers. The SUD also calculates version dependencies and conflicts to generate safe update lists. The SUD contains roles that represent entities inside the SUD with different responsibilities; when a role writes metadata it always signs it with its own key(s). The roles are: targets---stores the various updates' information; snapshot---creates metadata describing stable software bundles; timestamp---responsible for applying timestamps to targets' and snapshot's metadata, which is used to know if there are new updates; and root---acts as a Certification Authority (CA) for the other roles.

\textbf{Image Repository (IR).} This is a database where all OEM-associated software is stored, including packages developed in-house and from \textit{N}-Tier suppliers.

\textbf{The Update Distribution Broker (UDB).} The OEM's UDB manages publisher/subscriber relations.

\textbf{EV Station Manager (ESM).} The ESM manages a distributed network of vehicle update stations (UStations), e.g., associated with EV charging stations. The ESM acts as a CA for its stations, so the vehicles can attest the owner of each UStation. Each UStation collects identifiers about vehicle models in its corresponding zone, for which updates are downloaded and cached. The UStation pulls from the UE updates corresponding to the identifier, that by its turn subscribes to the corresponding updates provided by the manufacturer's SUD, through the MQTT pub/sub protocol. The UE then redirect the update downloads to the designated UStation. The UE can optimize the cache of the software updates on zonal-basis. It can also predict update usage, i.e., if an update $\Delta$ becomes available for a vehicle type that is frequently seen in its UStations, then it can preemptively publish it.

\textbf{Vehicle.} The vehicles are composed of a primary and several secondary ECUs, for which software updates are continuously needed. The vehicle learns about new updates only by querying the OEM's SUD. The software images can downloaded via the OEM's IR or through the UStations for faster and more efficient bandwidth utilization. 

\textbf{Supplier.} The suppliers produce and package the update images of each autopart, tag them by model and manufacturer, and store them in local or manufacturer's Image Repository. As explained later, a direct supplier (called Tier 1) can securely delegate software to other third-party (Tier 2 or Tier 3) suppliers.

\textbf{Time server.} There is a trusted source of time for all elements considered.

\subsection{Update initialization and publishing}

\subsubsection{Initialization}
Before dispatching a vehicle to the market, an OEM installs the most recent software versions for all of its parts. The vehicle's model and parts are known by its unique \textit{Vehicle Identification Number (VIN)}, composed of 17 characters. In particular, the very first 11 characters, we call them \textit{Model Identification Number (MIN)}, defines the corresponding features, specifications, and manufacturer. To keep the vehicle in circulation up-to-date, the OEM retains update's meta-data in the SUD's fleet inventory, namely:
\begin{itemize}
    \item The VIN,
    \item The MIN and a list of soft parts with associated suppliers, and
    \item The software update info.: last available version, associated package dependencies and conflicts, and packaging time.
\end{itemize}
We also assume the vehicle owner previously obtained a software update service account from the OEM to maintain its vehicle up-to-date.

\subsubsection{Update publishing}
Once a new update is ready to be made available for use, the protocol presented in Table~\ref{tab:update_steps}, and described in the following paragraphs.

\begin{table}[b]
    \caption{Update publishing steps.}
    \label{tab:update_steps}
    \centering
    \begin{tabular}{c|c}
    \toprule
        a) & OEM or supplier store update on IR \\
        b) & OEM or supplier provides update metadata to SUD \\
        c) & SUD informs UDB \\
        d) & UDB publishes to subscribers \\
        e) & Subscribers retrieve updates from IR \\
        f) & Subscribers place updates on the edge \\
        \bottomrule
    \end{tabular}
\end{table}


\textbf{a):} When a new software update $\Delta$ is ready to be deployed, the development team $dev$ places in the OEM's IR $\Delta$ and a manifest $X=(PB,\langle PB\rangle_{dev})$, where $PB=((f_\Delta,l_\Delta,h_\Delta,v_\Delta,e,d,cf),(t,v,r_{dev}))$.\\
\textit{Delegations.} When $\Delta$ is developed by a supplier, a delegation is created; the OEM stores some $\Delta$ that it did not developed, will sign manifests that mention $\Delta$ and its metadata, but the responsible for $\Delta$ and all security around it is the supplier.

\textbf{b):} Once the IR receives the manifest $X$, it pushes it into the SUD so it uses this information to update its inventory, conflicts, and roles.

\textbf{c):} The SUD informs the UBD there is an update available for the fleet.

\textbf{d):} The UDB informs its subscribers there is a new update to be fetched, \textit{e.g.}, the ESM.

\textbf{e):} The ESM queries the IR for updates.
The IR creates a new manifest $X$ where it add $r_{ESM}$ to the $PB$ block created in step \textbf{a)}, resulting in $X=(PB,\langle PB\rangle_{IR})$, where $PB=((f_\Delta,l_\Delta,h_\Delta,v_\Delta,e,d,cf,r_{ESM}),(t,v,r_{IR}))$.
This manifest allows the vehicles to know the IR vouches for this ESM to distribute $\Delta$, and subsequently, its charging stations.
The stations manager downloads this last manifest together with $\Delta$.

\textbf{f):} The EV stations manager distributes the update to the stations, who can now serve it directly to connected vehicles.

\subsection{Update Protocol}
In Table~\ref{tab:update_protocol} is presented the protocol the vehicles follow to get updates from the OEM, and described in the following.

\begin{table}[t]
    \caption{Vehicle update protocol.}
    \label{tab:update_protocol}
    \centering
    \begin{tabular}{c|c}
    \toprule
        1) & Connect to EV and authenticate UStation \\
        2) & Query SUD \\
        3) & Get updates from UStations \\
        4) & UStation cache management \\
    \bottomrule
    \end{tabular}
\end{table}

\textbf{0):} The vehicle's primary ECU preemptively starts the update process by building a version report manifest $X=(PB,\langle PB\rangle_{primary})$, where $PB=([(f_\Delta,l_\Delta,h_\Delta,v_\Delta,e)],(nonce,t,v,r_{primary}))$.
This manifest describes the current software versions of all ECUs in the vehicle.
This manifest is uploaded to the SUD, which identifies which packages the primary should download, and sends a tailored manifest $X$ describing only what the primary should download, where $X$ has the same structure of the manifest mentioned above.
Note that both manifests include a \emph{nonce} to prevent rollback attacks---all nonces used and received are saved by both parties.

\textbf{1):} The vehicle connects to an EV station for charging. At this point, the vehicle tries to interface with it via WiFi, powerline, or other communication medium available.
If there is an interaction, the vehicle will attempt to identify if this station is an update distribution point by authenticating it.

\textbf{2):} Once authenticated, the vehicle can continue the update protocol; if step 0) has not been performed yet, the vehicles does it now.
If there are updates to install, go to step 3); otherwise, abort the procedure.

\textbf{3):} Following the SUD's manifest, the vehicle queries the UStation for the update files.
There are three cases: update Hit, Miss, or Unknown.\\
\textit{Hit:} the UStation has local caches for the required updates.
This means that the UDB pushed the updates to this UStation, or that a previous access to this UStation had occurred by a vehicle requiring the same software. The vehicle's primary then downloads the software packages (i.e., all dependencies) of the software updates to be installed.\\
\textit{Miss:} the UStation does not have the packages requested by the vehicle. In this case, the UStation will pull updates from the UE. The UE sends an update link to download the update from the corresponding Image Repository. The UE sends a security token each time a download is requested by a UStation.\\
\textit{Unknown:} the current vehicle MID is unknown to the UStation $S$, i.e., have not been seen before. In this case, the UStation sends a subscribe request to the UE. If the latter has the MID subscription through another UStation $Z$ it adds $S$ to its list of destinations and pushes updates about this MID as above (by sending a download link and corresponding credentials). On the other hand, if the UE does not know about the MID at all, it subscribes to the OEM's SUD and starts getting meta-data updates about this model. This meta-data is then used to pull updates from Image Repositories as above.\\
By the end of this step, the primary should have downloaded all updates and corresponding manifests.
At this point, the primary performs a full verification, which is a procedure where the downloaded updates are checked against the downloaded metadata.
We describe this procedure in Section~\ref{sec:verification}.

\subsubsection{Pushing updates to Secondaries}
Pushing update from primaries to secondaries is key in automotive software updates. The role of a primary is essential in the process since the corresponding ECU has typically higher capacity (memory, bandwidth, and processing) than secondary constrained ECUs. On the other hand, given that a modern vehicle can have more than 100 ECUs, having each handling the update independently with the OEM SUD would be a very complex and costly task. Given this, there are two cases for pushing the updates from the primary to a secondary ECU considering the trust model.

\textbf{Trusted Primary.} Assuming the primary is trusted, it can handle the entire software download process, full verification (as specified in Section~\ref{sec:verification}), and delivery to the secondary ECU. The secondary on the other hand can have (1) a software update/flashing tool that could be executed directly remotely by the primary (e.g., in an RPC style), or (2) a running a flashing service process that can be invoked to the the update and flashing locally. In either case, the secondary does not have to verify the received updates via the trusted primary (although it should do a basic sanity check, e.g., error correction or erasure code). It would rather do a partial verification (as explained in Section~\ref{sec:verification}).

\textbf{Untrusted Primary.} An untrusted primary may lead to integrity or availability issues (and confidentiality if considered). It could violate integrity by forging the software update packages (i.e., updates and manifests). This would require the secondary to do a full verification for the updates. On the other hand, the primary may simply delay or drop the updates destined to the secondary. To address this, a secondary's flashing service (i.e., periodic process) should handle the communication with the primary, which can no longer enforce update remotely. The flashing service has two main roles. The first is to request an \textit{update report} from the primary upon each vehicle ignition. The primary should reply (within a given time delay) with a signed message from the OEM, specifying the last available software version for the corresponding secondary ECU. These two roles ensure that the primary could neither delay or discard the received updates from the OEM beyond the pre-defined period (e.g., defined on safety basis), nor tampering with their content. If these conditions are unmet, the secondary sends an alert message to the driver or OEM, e.g., via displaying an alert message on the headset or beeping. 

QUESTION: after pushing, there is flashing. If some ECU failed and there are dependencies, there others should roll-back. This needs some atomic broadcast protocol to be done well. What is your take?

\subsection{Extensions}
\subsubsection{Adding/removing a UStation}
The UDB should be able to scale-out and scale-in over time. This is done by adding new UStations or removing others occasionally or permanently, e.g., in the case of a "retired" UStation. The main incentives are referred to business, convenience, and performance reasons. Nevertheless, denouncing some UStations may be driven by security threats which requires putting the UStation out of service. 

Technically, when adding a new UStation, it gets assigned an identifier and a security authentication key, i.e., a certificate. This is needed to ensure that the vehicles authenticate to approved and trusted UStations, through which software updates are downloaded. A UStation that is under threat can get its certificate revoked and the key is added to the UDB Certificate Revocation List (CRL), that is always updated and sent to the vehicles. Vehicles are then protected since software updates can no longer be validated. 

\subsubsection{Incremental updates}
In modern vehicles, the software update footprint can be very large (e.g., up to 1 GB). In this case, not all updates are expected to be fully downloaded at a UStation. To the contrary, the vehicle should be able to continue downloading the update remainder (to reduce bandwidth, time, and energy waste) through other means, e.g., another UStation or directly through the OEM via a cellular or 5G connection. For this, updates can be packaged as a series of fine-grained ordered \textit{buckets}. A download that is interrupted at some bucket could easily continue the download from the failed bucket forward, until the complete package is downloaded. The primary verifies this after the download is complete by checking the digest of the the full package across the assembled one of the ordered buckets downloaded. This ensures that no buckets but the correct ones are added in their specific order.   

\subsubsection{Reducing Misses}

One of the properties of \acronym is reducing the update time. This is salient in the case of cache hit since the update is at the closest proximity to the vehicle. However, under cache hits, the update time will be higher since the UStation should get the update throughout the UDB while the vehicle is waiting for the update at the station.
While having a decent cache storage capacity can reduce the cache misses, software update cannot be afforded at scale. On the other hand, a newly added UStation would suffer a lot of cache misses. 

To address this, we propose a proactive technique to speculate the needed updates at a new UStation A or pushing updates for new vehicles even if they have not been requested by an existing UStation. This technique is based on filling A's cache using the cache of the k $l$-hop closest UStations, where $l \in \mathbb{N}$. The intuition is that it is likely that vehicle models circulating in the proximity of A are significantly similar to those already passed by the neighbouring k USations. Therefore, the UDB engine UE computes a list of the cardinally of the MIDs at the k UStations. The highest the cardinally the more abundant a associated model is in a zone. The UE then sends the list to  UStation A that proactively initiates downloading the updates starting with the the highest carnality MIDs, and until the cache is full. Although this technique improves the hit rate much better than an empty cache, an interesting research is to study more intelligent ML-based recommender systems, based on the traffic at the neighbours and trajectories patterns.







==> discuss.tex <==
\section{Feasibility Discussion}
\label{sec:discuss}
While the need for building resilient systems is very well understood, applying redundancy-based solutions like IRS may look infeasible for in-vehicular systems. 
%(Indeed, the authors of this paper had this old belief as well a decade ago.) 
Nevertheless, we argue that this is no longer the case as the three trends automation, digitization, and connectivity have changed modern vehicular systems dramatically. In this section, we try to alleviate these concerns by driving a conceptual analysis demonstrating the feasibility of IRS to modern vehicles.

\subsection{Distributed and Redundant Applications}
The current application landscape in automotive is very rich and complex, spanning ADAS \& Safety Systems, Infotainment, Body Electronics, Powertrain, and Telematics. At a fine-grained level, these applications incur millions of functionalities. For instance, a Volvo modern vehicle ``contains 10 million conditional statements as well as 3 million functions, which are invoked some 30 million places in the source code''~\cite{sw-eat-car:2021}. Many of these applications are becoming naturally distributed across the vehicle to manage the dependencies between functionalities and to synchronize the similar ones across the vehicle. For instance, a vehicle may have applications running four steering, braking, tyre pressure processes; four/five door lock and window processes; four light sets of processes, two mirror processes, several airbag processes, etc. Nevertheless, these processes are currently only synchronized in a passive  way, i.e., propagating notifications, where ``decisions'', e.g., changing an actuator state, are only made locally. Given this, the overhead of enforcing distributed control through agreement protocols prior to changing the application state would be reasonably low. This is sound for safety/security critical applications that are soft-real time, in particular, like door lock/unlock, window open/close, and OTA update validation by different processes on different ECUs. %Notice that these applications do not have strict latency requirements, and thus IRS is likely to be a valid option more than other real-time applications that may not afford the agreement delays.

\subsection{Distributed Architecture}
The vehicular architecture is becoming heavily distributed as more ECUs are being added over time to cope with the application demands. Considering the evolution of distributed architectures~\cite{auto-market-mckinsey:2019}, applications are becoming more aggregated in larger ECUs: (1) Domain-based ones aggregate applications with similar functionalities; (2) Zonal-based ones aggregate based on the vehicle zone, e.g., a Door Control Unit hosts many applications (like door locks, motors, windows, theme lights) at the door proximity; and (3) Centralized. The former two are considered very convenient environments to run replicated protocols as the agreement protocol suggested in IRS. In addition, multiple aggregated applications can directly benefit from the IRS being a middleware/service. Indeed, while the replication cost has always been an adoption barrier in the IT world, the costs (surprisingly) look lower in vehicular architectures being natively distributed. The latter centralized architecture is estimated to appear in the future, although it is a weak design from a security perspective, being a single point of failure/attack. To this end, transforming the central controller into a distributed cluster can mitigate the risk significantly.

\subsection{Efficient and Secure Networks}
Vehicular networks, especially the CAN bus, have always been considered slow and the weakest spot in a vehicle. In particular, the classical baud rate of CAN bus cannot be higher than 1Mbps, and the payload is only 8 bytes per packet\footnote{The CAN bus is a broadcast-based network that arbitrates message identifiers on a bit basis. The lower the identifier (composed of a number of bits, e.g., 11 bits) the highest its priority. In this sense, a competing message with lowest identifier can take over sending over the bus. This imposes limits on payload sizes to maintain high message frequencies.}. 
This prohibits an IRS-like solution where the agreement meta-data (identifiers, signatures, cryptographic digests, clock) is high. On the other hand, CAN frames lack the sender/receiver identifiers which makes  authentication and integrity a non-trivial task. However, the new versions of CAN, i.e., CAN FD and XL, have larger frame's payload size of 64B and 2KB, and baud rate to 2Mbps and 10Mbps, respectively. Furthermore, novel networks like Automotive Ethernet and FlexRay have native security support and an order of magnitude higher bit rate. We believe that these advancements mitigate the concerns regarding the feasibility of IRS to such environment.

\subsection{Decent HW/SW Stack}
It can be assumed that running IRS agreement protocols in a constrained device, like a micro-controller-based ECU, would be an overkill due to the heavy use of cryptography. However, modern automotive ECUs (microprocessor-based and multi-core) are getting high computational and storage capacities that could be compared to a Raspberry Pi or a mobile phone\footnote{https://www.emobility-engineering.com/focus-ecus/}. This is correct, in particular, for main ECUs like domain and zone controllers, gateways, telecommunication units, etc. On top of this hardware, the software stack~\cite{e2e-market-mckinsey:2020} is also getting more mature while we observe more UNIX, POSIX, and Linux-based RTOS/OS, e.g., AGL, RTLinux, QNX, Android Auto, and Apple CarPlay. This also means that a lot of IT/IoT libraries can now be adapted or used in automotive. New architectures are widely adopting the virtualization hypervisor technology, which facilitates application deployments on an ECU, and thus, replication in our case~\cite{e2e-market-mckinsey:2020}. Therefore, the modern HW/SW stack of modern vehicles is decent enough to support a solution like IRS.





